A Deep-Learning Framework for Improving COVID-19 CT Image Quality and Diagnostic Accuracy

We present a deep-learning based computing framework for fast-and-accurate CT (DL-FACT) testing of COVID-19. Our CT-based DL framework was developed to improve the testing speed and accuracy of COVID-19 (plus its variants) via a DL-based approach for CT image enhancement and classification. The image enhancement network is adapted from DDnet, short for DenseNet and Deconvolution based network. To demonstrate its speed and accuracy, we evaluated DL-FACT across several sources of COVID-19 CT images. Our results show that DL-FACT can significantly shorten the turnaround time from days to minutes and improve the COVID-19 testing accuracy up to 91%. DL-FACT could be used as a software tool for medical professionals in diagnosing and monitoring COVID-19.

==> table/2d_3d_comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\caption{Summary of operations used in 2D and 3D CNN}
\label{tab:2d_3d_comp}
\begin{threeparttable}
\begin{tabular}{|l|r|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Operation}}                                        & \multicolumn{1}{c|}{\textbf{Version}} & \multicolumn{1}{c|}{\textbf{Defiition}} \\ \hline
\multirow{2}{*}{Convolution}                                                    & 2D                                    & \begin{tabular}[c]{@{}c@{}}
                              \(\displaystyle output(x, y, z) 
                                = 
                                bias(z) + 
                                \sum_{z_i=0}^{Z_i}  
                                \sum_{i=0}^{f\_size}
                                \sum_{j=0}^{f\_size} \)
                                \\\(\displaystyle input(x+i, y+j, z_i) \times filter(i, j, z, z_i)\)
                                \end{tabular}                  \\ \cline{2-3} 
                                                                                & 3D                                    &  
                              \begin{tabular}[c]{@{}c@{}}
                              \(\displaystyle output(w, x, y, z) 
                                = 
                                bias(z) + 
                                \sum_{z_i=0}^{Z_i}  
                                \sum_{i=0}^{f\_size}
                                \sum_{j=0}^{f\_size} 
                                \sum_{k=0}^{f\_size}\)
                                \\\(\displaystyle input(w+i, x+j, y+k, z_i) \times filter(i, j, k, z, z_i)\)
                                \end{tabular} 
                            
                                \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Non-linear\\ activation \\ (Leaky-relu)\end{tabular}}                                                     & 2D                                    & 
                                \begin{tabular}[c]{@{}c@{}}
                              \(\displaystyle 
                              output(x,y,z)= 
                                \begin{cases}
                                    input(x, y, x)          & \text{if } input(x, y, z)\geq 0\\    
                                    0.1 \times input(x, y, z)     & \text{otherwise}
                                \end{cases}
                              \)
                                \end{tabular}
                   \\ \cline{2-3} 
                                                                                & 3D                                    &    
                                \begin{tabular}[c]{@{}c@{}}
                              \(\displaystyle 
                              output(w,x,y,z)= 
                                \begin{cases}
                                    input(w, x, y, x)          & \text{if } input(w, x, y, z)\geq 0\\    
                                    0.1 \times input(w, x, y, z)     & \text{otherwise}
                                \end{cases}
                              \)
                                \end{tabular}                                                
                                                                                \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Batch-\\ normalization\tnote{*}\end{tabular}} & 2D                                    & 
                            \begin{tabular}[c]{@{}c@{}}
                              \(\displaystyle 
                              output(x, y, z) 
                                = 
                                    \frac{input(x, y, z) - E(z)}{\sqrt{Var(z) + \epsilon}}
                                    \times \alpha + \beta
                              \)
                                \end{tabular}
                                
                                \\ \cline{2-3} 
                                                                                & 3D                                    &    
                                \begin{tabular}[c]{@{}c@{}}
                              \(\displaystyle 
                              output(w, x, y, z) 
                                = 
                                    \frac{input(w, x, y, z) - E(z)}{\sqrt{Var(z) + \epsilon}}
                                    \times \alpha + \beta
                              \)
                                \end{tabular}
                                                                                \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Pooling \\ (Max pool)\end{tabular}}                                                        & 2D                                    & 
                            \begin{tabular}[c]{@{}l@{}}
                              \(\displaystyle 
                              output(x, y, z) =
                              \) \\
                              \(\displaystyle 
                               \max_{\{i=0..f\_size-1, j=0..f\_size-1\}} input(x+i, y+j, z)
                              \)
                                \end{tabular}                  \\ \cline{2-3} 
                                                                                & 3D                                    & 
                            \begin{tabular}[c]{@{}l@{}}
                              \(\displaystyle 
                              output(w, x, y, z) =
                              \) \\
                              \(\displaystyle 
                               \max_{\{i=0..f\_size-1, j=0..f\_size-1, k=0..f\_size-1\}} input(w+i, x+j, y+k, z)
                              \)
                                \end{tabular} 
                                                                                \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Pooling \\ (Linear)\end{tabular}}                                                        & 2D                                    & \begin{tabular}[c]{@{}l@{}}
                              \(\displaystyle 
                              output(x, y) 
        = f(x_2, y_2) \times \frac{(x_2 – x)}{(x_2 – x_1)} + f(x_1, y_1) \times \frac{(x – x_1))}{(x_2 – x_1)}
                              \)
                                \end{tabular}                    \\ \cline{2-3} 
                                                                                & 3D                                    &   
                                \begin{tabular}[c]{@{}l@{}}
                              \(\displaystyle 
                              output(x, y, z) = 
        f(x_2, y_2, z_2) \times \frac{(x_2 – x)}{(x_2 – x_1)} + f(x_1, y_1, z_1) \times \frac{(x – x_1))}{(x_2 – x_1)}
                              \)
                                \end{tabular}
                                                                                \\ \hline
\multirow{2}{*}{Deconvolution}                                                        & 2D                                    & Algorithm  \ref{alg: 2d_deconv}                  \\ \cline{2-3} 
                                                                                & 3D                                    &    Algorithm \ref{alg: 3d_deconv}                                     \\ \hline
\end{tabular}
\begin{tablenotes}\footnotesize
\item[*] E[x] and Var[x] represent the mean and standard deviation of the inputs, respectively. $\alpha$ and $\beta$ are the learnable parameters. These parameters are constant in the trained network.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> table/computecovid19_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{Comparison of ComputeCOVID19+ with existing similar work}
\label{tab:computecovid19_comparison}
\begin{threeparttable}
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Framework}}}                                                       & \multicolumn{2}{c|}{\textbf{CT scans pre-processing}}                                                                        & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}3D/2D \\ classification\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Data \\ labeling \end{tabular}}} &  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Supported hardware for\\ inference\end{tabular}}} \\ \cline{2-3} \cline{6-8} 
\multicolumn{1}{|c|}{}                                                                                          & \begin{tabular}[c]{@{}c@{}}Image \\enhancement\end{tabular} & \begin{tabular}[c]{@{}c@{}}Image \\segmentation\end{tabular} &            &                                                                               & ~\hspace{0.07cm}CPU~\hspace{0.07cm}             & ~\hspace{0.07cm}GPU~\hspace{0.07cm}                               & FPGA                      \\ \hline
ComputeCOVID19+                                                                                                 & \color{green}$\checkmark$                                                            & \color{green}$\checkmark$                                                             & 3D   &   Not required                                                                                  & \color{green}$\checkmark$                                 & \color{green}$\checkmark$                                 & \color{green}$\checkmark$
%\textsuperscript{1}  
\\ \hline
\begin{tabular}[c]{@{}l@{}}He et al.~\cite{he2020sample}\end{tabular}                  & \color{red}$\times$                                                            & \color{red}$\times$                                                             & 2D     &  Manual\textsuperscript{2}                                                                                  & \color{green}$\checkmark$                                 & \color{green}$\checkmark$                                 & \color{red}$\times$                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}M-inception~\cite{wang2020deep}\end{tabular} & \color{red}$\times$                                                            & \color{green}$\checkmark$                                                             & 2D   &  Manual\textsuperscript{2}                                                                                   & *                                & *                                 & \color{red}$\times$                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}DRE-Net~\cite{song2020deep}\end{tabular}     & \color{red}$\times$                                                            & \color{green}$\checkmark$                                                             & 2D    &  Manual\textsuperscript{2}                                                                                  & *                                 & *                                 & \color{red}$\times$                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}Li et al.~\cite{li2020using}\end{tabular}                   & \color{red}$\times$                                                            & \color{green}$\checkmark$                                                             & 2D    &  Manual\textsuperscript{2}                                                                                 & *                                 & \color{green}$\checkmark$                                 & \color{red}$\times$                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}DeCoVNet~\cite{zheng2020deep}\end{tabular}  & \color{red}$\times$                                                            & \color{green}$\checkmark$                                                             & 3D     &  Not required                                                                                 & *                                 & \color{green}$\checkmark$                                 & \color{red}$\times$                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}Harmon et al.~\cite{Harmon2020}\end{tabular}                & \color{red}$\times$                                                            & \color{green}$\checkmark$                                                             & 3D     &  Not required                                                                                 & \color{red}$\times$                                 & \color{green}$\checkmark$                                 & \color{red}$\times$                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}Serte et al.~\cite{serte2021deep}\end{tabular}              & \color{red}$\times$                                                            & \color{red}$\times$                                                             & 2D/3D      &    Not required                                                                           & *                                 & \color{green}$\checkmark$                                 & \color{red}$\times$                                 \\ \hline
\end{tabular}
\begin{tablenotes}\footnotesize
\item[*]No information available.
%\item[\textsuperscript{1} ]Support for enhancement AI is tested and evaluated on Intel$^{\circledR}$ Arria-10 FPGA. The implementation could be easily ported to other AIs. However, sice the source code of classification and segmentation AI is not available, they are not tested on FPGA.
\item[\textsuperscript{2} ]CT images showing symptoms of COVID-19 must be manually filtered.
\end{tablenotes}
\end{threeparttable}
\end{table*}

==> table/data_source.tex <==
\begin{table}[]
\caption{Data source description}
\label{tab:data_source}
\scalebox{0.9}{
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Data source}}                                                            & \multicolumn{1}{c|}{\textbf{Contents}}                                                                                                              \\ \hline
Mayo Clinic                                                                                       & \begin{tabular}[c]{@{}l@{}}Eight (8) healthy chest CT scans \\ and associated projection data at \\ full-dose \& quarter-dose radiation\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Medical Imaging \\ Databank of the \\ Valencia Region (BIMCV)\end{tabular} & \begin{tabular}[c]{@{}l@{}}X-ray scans and CT scans of \\ 34 COVID-19 patients\end{tabular}                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}Medical Imaging and \\ Data Resource Center \\ (MIDRC)\end{tabular}        & \begin{tabular}[c]{@{}l@{}}229 CT scans of COVID-19 patients \end{tabular}                                                               \\ \hline
\begin{tabular}[c]{@{}l@{}}Lung Image Database \\ Consortium Image \\ Collection (LIDC)\end{tabular}  & 1301 healthy chest CT scans                                                                                                                         \\ \hline
\end{tabular}
}
\vspace{-9pt}
\end{table}

==> table/ddnet_layers.tex <==
\begin{table*}[!htb]
\huge
\caption{Input and output sizes and filter size of feature maps for the convolution and deconvolution layers in DDnet}
\label{tab:dd_net_feature_maps}
\scalebox{0.475}{
\begin{tabular}{lllllllllllll}
\hline
\multicolumn{1}{|l|}{\textbf{Layer}}       & \multicolumn{1}{l|}{1}                        & \multicolumn{1}{l|}{2}                        & \multicolumn{1}{l|}{3}                        & \multicolumn{1}{l|}{4}                        & \multicolumn{1}{l|}{5}                        & \multicolumn{1}{l|}{6}                        & \multicolumn{1}{l|}{7}                        & \multicolumn{1}{l|}{8}                        & \multicolumn{1}{l|}{9}                        & \multicolumn{1}{l|}{10}                       & \multicolumn{1}{l|}{11}                       & \multicolumn{1}{l|}{12}                       \\ \hline
\multicolumn{1}{|l|}{\textbf{Kernels}}      & \multicolumn{1}{l|}{conv1}                    & \multicolumn{1}{l|}{conv2}                    & \multicolumn{1}{l|}{conv3}                    & \multicolumn{1}{l|}{conv4}                    & \multicolumn{1}{l|}{conv5}                    & \multicolumn{1}{l|}{conv6}                    & \multicolumn{1}{l|}{conv7}                    & \multicolumn{1}{l|}{conv8}                    & \multicolumn{1}{l|}{conv9}                    & \multicolumn{1}{l|}{conv10}                   & \multicolumn{1}{l|}{conv11}                   & \multicolumn{1}{l|}{conv12}                   \\ \hline
\multicolumn{1}{|l|}{\textbf{Input size}}  & \multicolumn{1}{l|}{512$\times$512$\times$1}  & \multicolumn{1}{l|}{256$\times$256$\times$16} & \multicolumn{1}{l|}{256$\times$256$\times$64} & \multicolumn{1}{l|}{256$\times$256$\times$32} & \multicolumn{1}{l|}{256$\times$256$\times$64} & \multicolumn{1}{l|}{256$\times$256$\times$48} & \multicolumn{1}{l|}{256$\times$256$\times$64} & \multicolumn{1}{l|}{256$\times$256$\times$64} & \multicolumn{1}{l|}{256$\times$256$\times$64} & \multicolumn{1}{l|}{256$\times$256$\times$80} & \multicolumn{1}{l|}{128$\times$128$\times$16} & \multicolumn{1}{l|}{128$\times$128$\times$64} \\ \hline
\multicolumn{1}{|l|}{\textbf{Output size}} & \multicolumn{1}{l|}{512$\times$512$\times$16} & \multicolumn{1}{l|}{256$\times$256$\times$64} & \multicolumn{1}{l|}{256$\times$256$\times$16} & \multicolumn{1}{l|}{256$\times$256$\times$64} & \multicolumn{1}{l|}{256$\times$256$\times$16} & \multicolumn{1}{l|}{256$\times$256$\times$64} & \multicolumn{1}{l|}{256$\times$256$\times$16} & \multicolumn{1}{l|}{256$\times$256$\times$64} & \multicolumn{1}{l|}{256$\times$256$\times$16} & \multicolumn{1}{l|}{256$\times$256$\times$16} & \multicolumn{1}{l|}{128$\times$128$\times$64} & \multicolumn{1}{l|}{128$\times$128$\times$16} \\ \hline
\multicolumn{1}{|l|}{\textbf{\textbf{Filter size}}} & \multicolumn{1}{l|}{7$\times$7}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               \\ \hline
                                  &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               \\ \hline
\multicolumn{1}{|l|}{\textbf{Layer}}       & \multicolumn{1}{l|}{13}                       & \multicolumn{1}{l|}{14}                       & \multicolumn{1}{l|}{15}                       & \multicolumn{1}{l|}{16}                       & \multicolumn{1}{l|}{17}                       & \multicolumn{1}{l|}{18}                       & \multicolumn{1}{l|}{19}                       & \multicolumn{1}{l|}{20}                       & \multicolumn{1}{l|}{21}                       & \multicolumn{1}{l|}{22}                       & \multicolumn{1}{l|}{23}                       & \multicolumn{1}{l|}{24}                       \\ \hline
\multicolumn{1}{|l|}{\textbf{Kernels}}      & \multicolumn{1}{l|}{conv13}                   & \multicolumn{1}{l|}{conv14}                   & \multicolumn{1}{l|}{conv15}                   & \multicolumn{1}{l|}{conv16}                   & \multicolumn{1}{l|}{conv17}                   & \multicolumn{1}{l|}{conv18}                   & \multicolumn{1}{l|}{conv19}                   & \multicolumn{1}{l|}{conv20}                   & \multicolumn{1}{l|}{conv21}                   & \multicolumn{1}{l|}{conv22}                   & \multicolumn{1}{l|}{conv23}                   & \multicolumn{1}{l|}{conv24}                   \\ \hline
\multicolumn{1}{|l|}{\textbf{Input size}}  & \multicolumn{1}{l|}{128$\times$128$\times$32} & \multicolumn{1}{l|}{128$\times$128$\times$64} & \multicolumn{1}{l|}{128$\times$128$\times$48} & \multicolumn{1}{l|}{128$\times$128$\times$64} & \multicolumn{1}{l|}{128$\times$128$\times$64} & \multicolumn{1}{l|}{128$\times$128$\times$64} & \multicolumn{1}{l|}{128$\times$128$\times$80} & \multicolumn{1}{l|}{64$\times$64$\times$16}   & \multicolumn{1}{l|}{64$\times$64$\times$64}   & \multicolumn{1}{l|}{64$\times$64$\times$32}   & \multicolumn{1}{l|}{64$\times$64$\times$64}   & \multicolumn{1}{l|}{64$\times$64$\times$48}   \\ \hline
\multicolumn{1}{|l|}{\textbf{Output size}} & \multicolumn{1}{l|}{128$\times$128$\times$64} & \multicolumn{1}{l|}{128$\times$128$\times$16} & \multicolumn{1}{l|}{128$\times$128$\times$64} & \multicolumn{1}{l|}{128$\times$128$\times$16} & \multicolumn{1}{l|}{128$\times$128$\times$64} & \multicolumn{1}{l|}{128$\times$128$\times$16} & \multicolumn{1}{l|}{128$\times$128$\times$16} & \multicolumn{1}{l|}{64$\times$64$\times$64}   & \multicolumn{1}{l|}{64$\times$64$\times$16}   & \multicolumn{1}{l|}{64$\times$64$\times$64}   & \multicolumn{1}{l|}{64$\times$64$\times$16}   & \multicolumn{1}{l|}{64$\times$64$\times$64}   \\ \hline
\multicolumn{1}{|l|}{\textbf{Filter size}} & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               \\ \hline
                                  &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               \\ \hline
\multicolumn{1}{|l|}{\textbf{Layer}}       & \multicolumn{1}{l|}{25}                       & \multicolumn{1}{l|}{26}                       & \multicolumn{1}{l|}{27}                       & \multicolumn{1}{l|}{28}                       & \multicolumn{1}{l|}{29}                       & \multicolumn{1}{l|}{30}                       & \multicolumn{1}{l|}{31}                       & \multicolumn{1}{l|}{32}                       & \multicolumn{1}{l|}{33}                       & \multicolumn{1}{l|}{34}                       & \multicolumn{1}{l|}{35}                       & \multicolumn{1}{l|}{36}                       \\ \hline
\multicolumn{1}{|l|}{\textbf{Kernels}}      & \multicolumn{1}{l|}{conv25}                   & \multicolumn{1}{l|}{conv26}                   & \multicolumn{1}{l|}{conv27}                   & \multicolumn{1}{l|}{conv28}                   & \multicolumn{1}{l|}{conv29}                   & \multicolumn{1}{l|}{conv30}                   & \multicolumn{1}{l|}{conv31}                   & \multicolumn{1}{l|}{conv32}                   & \multicolumn{1}{l|}{conv33}                   & \multicolumn{1}{l|}{conv34}                   & \multicolumn{1}{l|}{conv35}                   & \multicolumn{1}{l|}{conv36}                   \\ \hline
\multicolumn{1}{|l|}{\textbf{Input size}}  & \multicolumn{1}{l|}{64$\times$64$\times$64}   & \multicolumn{1}{l|}{64$\times$64$\times$64}   & \multicolumn{1}{l|}{64$\times$64$\times$64}   & \multicolumn{1}{l|}{64$\times$64$\times$80}   & \multicolumn{1}{l|}{32$\times$32$\times$16}   & \multicolumn{1}{l|}{32$\times$32$\times$64}   & \multicolumn{1}{l|}{32$\times$32$\times$32}   & \multicolumn{1}{l|}{32$\times$32$\times$64}   & \multicolumn{1}{l|}{32$\times$32$\times$48}   & \multicolumn{1}{l|}{32$\times$32$\times$64}   & \multicolumn{1}{l|}{32$\times$32$\times$64}   & \multicolumn{1}{l|}{32$\times$32$\times$64}   \\ \hline
\multicolumn{1}{|l|}{\textbf{Output size}} & \multicolumn{1}{l|}{64$\times$64$\times$16}   & \multicolumn{1}{l|}{64$\times$64$\times$64}   & \multicolumn{1}{l|}{64$\times$64$\times$16}   & \multicolumn{1}{l|}{64$\times$64$\times$16}   & \multicolumn{1}{l|}{32$\times$32$\times$64}   & \multicolumn{1}{l|}{32$\times$32$\times$16}   & \multicolumn{1}{l|}{32$\times$32$\times$64}   & \multicolumn{1}{l|}{32$\times$32$\times$16}   & \multicolumn{1}{l|}{32$\times$32$\times$64}   & \multicolumn{1}{l|}{32$\times$32$\times$16}   & \multicolumn{1}{l|}{32$\times$32$\times$64}   & \multicolumn{1}{l|}{32$\times$32$\times$16}   \\ \hline
\multicolumn{1}{|l|}{\textbf{Filter size}} & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               \\ \hline
                                  &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               &                                               \\ \cline{1-10}
\multicolumn{1}{|l|}{\textbf{Layer}}       & \multicolumn{1}{l|}{37}                      & \multicolumn{1}{l|}{38}                       & \multicolumn{1}{l|}{39}                       & \multicolumn{1}{l|}{40}                       & \multicolumn{1}{l|}{41}                       & \multicolumn{1}{l|}{42}                       & \multicolumn{1}{l|}{43}                       & \multicolumn{1}{l|}{44}                       & \multicolumn{1}{l|}{45}                       &                                               &                                               &                                               \\ \cline{1-10}
\multicolumn{1}{|l|}{\textbf{Kernels}}      & \multicolumn{1}{l|}{conv37}                   & \multicolumn{1}{l|}{deconv1}                  & \multicolumn{1}{l|}{deconv2}                  & \multicolumn{1}{l|}{deconv3}                  & \multicolumn{1}{l|}{deconv4}                  & \multicolumn{1}{l|}{deconv5}                  & \multicolumn{1}{l|}{deconv6}                  & \multicolumn{1}{l|}{deconv7}                  & \multicolumn{1}{l|}{deconv8}                  &                                               &                                               &                                               \\ \cline{1-10}
\multicolumn{1}{|l|}{\textbf{Input size}}  & \multicolumn{1}{l|}{32$\times$32$\times$80}   & \multicolumn{1}{l|}{64$\times$64$\times$32}   & \multicolumn{1}{l|}{64$\times$64$\times$32}   & \multicolumn{1}{l|}{128$\times$64$\times$32}  & \multicolumn{1}{l|}{128$\times$128$\times$32} & \multicolumn{1}{l|}{256$\times$256$\times$32} & \multicolumn{1}{l|}{256$\times$256$\times$32} & \multicolumn{1}{l|}{512$\times$512$\times$32} & \multicolumn{1}{l|}{512$\times$512$\times$32} &                                               &                                               &                                               \\ \cline{1-10}
\multicolumn{1}{|l|}{\textbf{Output size}} & \multicolumn{1}{l|}{32$\times$32$\times$16}   & \multicolumn{1}{l|}{64$\times$64$\times$32}   & \multicolumn{1}{l|}{64$\times$64$\times$16}   & \multicolumn{1}{l|}{128$\times$64$\times$32}  & \multicolumn{1}{l|}{128$\times$128$\times$16} & \multicolumn{1}{l|}{256$\times$256$\times$32} & \multicolumn{1}{l|}{256$\times$256$\times$16} & \multicolumn{1}{l|}{512$\times$512$\times$32} & \multicolumn{1}{l|}{512$\times$512$\times$1}  &                                               &                                               &                                               \\ \cline{1-10}
\multicolumn{1}{|l|}{\textbf{Filter size}} & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               & \multicolumn{1}{l|}{5$\times$5}               & \multicolumn{1}{l|}{1$\times$1}               &                                               &                                               &                                               \\ \cline{1-10}
\end{tabular}
}


\end{table*}

==> table/ddnet_layers1.tex <==
\begin{table}[]
\caption{Input and output sizes and filter size of feature maps for the convolution and deconvolution layers in DDnet}
\label{tab:dd_net_feature_maps1}
\scalebox{0.9}{
\begin{tabular}{|c|c|c|}
\hline
\textbf{Layers} & \textbf{Output Size} & \textbf{Details}          \\ \hline
Convolution 1   & 512$\times$512$\times$16           & filter size=7$\times$7, stride=1 \\ \hline
Pooling 1       & 256$\times$256$\times$16           & filter size=3$\times$3, stride=2 \\ \hline
Dense Block 1   & 256$\times$256$\times$80           & filter size=\begin{bmatrix} 1\times 1  \\ 5 \times 5  \\ \end{bmatrix} $\times$ 4, stride=1   \\ \hline
Convolution 2   & 256$\times$256$\times$16           & filter size=1$\times$1, stride=1 \\ \hline
Pooling 2       & 128$\times$128$\times$16           & filter size=3$\times$3, stride=2 \\ \hline
Dense Block 2   & 128$\times$128$\times$80           & filter size=\begin{bmatrix} 1\times 1  \\ 5 \times 5  \\ \end{bmatrix} $\times$ 4, stride=1   \\ \hline
Convolution 3   & 128$\times$128$\times$16           & filter size=1$\times$1, stride=1 \\ \hline
Pooling 3       & 64$\times$64$\times$16             & filter size=3$\times$3, stride=2 \\ \hline
Dense Block 3   & 64$\times$64$\times$80             & filter size=\begin{bmatrix} 1\times 1  \\ 5 \times 5  \\ \end{bmatrix} $\times$ 4, stride=1   \\ \hline
Convolution 4   & 64$\times$64$\times$16             & filter size=1$\times$1, stride=1 \\ \hline
Pooling 5       & 32$\times$32$\times$16             & filter size=3$\times$3, stride=2 \\ \hline
Dense Block 4   & 32$\times$32$\times$80             & filter size=\begin{bmatrix} 1\times 1  \\ 5 \times 5  \\ \end{bmatrix} $\times$ 4, stride=1   \\ \hline
Convolution 5   & 32$\times$32$\times$16             & filter size=1$\times$1, stride=1 \\ \hline
Un-pooling 1    & 64$\times$64$\times$16             & scale factor=2            \\ \hline
Deconvolution 1 & 64$\times$64$\times$32             & filter size=5$\times$5, stride=1 \\ \hline
Deconvolution 2 & 64$\times$64$\times$16             & filter size=1$\times$1, stride=1 \\ \hline
Un-pooling 2    & 128$\times$128$\times$16           & scale factor=2            \\ \hline
Deconvolution 3 & 128$\times$128$\times$32           & filter size=5$\times$5, stride=1 \\ \hline
Deconvolution 4 & 128$\times$128$\times$16           & filter size=1$\times$1, stride=1 \\ \hline
Un-pooling 3    & 256$\times$256$\times$16           & scale factor=2            \\ \hline
Deconvolution 3 & 256$\times$256$\times$32           & filter size=5$\times$5, stride=1 \\ \hline
Deconvolution 5 & 256$\times$256$\times$16           & filter size=1$\times$1, stride=1 \\ \hline
Un-pooling 4    & 512$\times$512$\times$16           & scale factor=2            \\ \hline
Deconvolution 6 & 512$\times$512$\times$32           & filter size=5$\times$5, stride=1 \\ \hline
Deconvolution 7 & 512$\times$512$\times$1            & filter size=1$\times$1, stride=1 \\ \hline
\end{tabular}
}
\vspace{-9pt}
\end{table}

==> table/den_121_arch.tex <==
\begin{table}[]
\centering
\caption{Architecture of 3D version of DenseNet 121}
\label{tab:den121_arch}
\scalebox{0.90}{
\begin{tabular}{c|c|c}
\hline \hline
\textbf{Layers}                       & \textbf{Ouput Size}             & \textbf{Details}                                                                                                  \\ \hline \hline
Convolution                           & 94 $\times$ 94 $\times$ 30               & 7 $\times$ 7 $\times$ 7 conv, stride 2                                                                             \\ \hline
Pooling                               & 46 $\times$ 46 $\times$ 14                 & 3 $\times$ 3 $\times$ 3 max pool, stride 2                                                                         \\ \hline
Dense Block 1                         & 46 $\times$ 46 $\times$ 14                 & \begin{bmatrix} 1\times 1\times 1 \text{ conv}  \\ 3 \times 3 \times 3 \text{ conv}  \\ \end{bmatrix} $\times$ 6   \\ \hline
\multirow{2}{*}{Transition Layer 1}   & 46 $\times$ 46 $\times$ 14                 & 1 $\times$ 1 $\times$ 1 conv                                                                                       \\ \cline{2-3} 
                                      & 23 $\times$ 23 $\times$ 7                 & 2 $\times$ 2 $\times$ 2 average pool, stride 2                                                                     \\ \hline
Dense Block 2                         & 23 $\times$ 23 $\times$ 7                 & \begin{bmatrix} 1\times 1\times 1 \text{ conv}  \\ 3 \times 3 \times 3 \text{ conv}  \\ \end{bmatrix} $\times$ 12  \\ \hline
\multirow{2}{*}{Transition Layer 2}   & 23 $\times$ 23 $\times$ 7                 & \begin{bmatrix} 1\times 1\times 1 \text{ conv}  \\ 3 \times 3 \times 3 \text{ conv}  \\ \end{bmatrix} $\times$ 6   \\ \cline{2-3} 
                                      & 12 $\times$ 12 $\times$ 4                 & 2 $\times$ 2 $\times$ 2 average pool, stride 2                                                                     \\ \hline
Dense Block 3                         & 12 $\times$ 12 $\times$ 4                 & \begin{bmatrix} 1\times 1\times 1 \text{ conv}  \\ 3 \times 3 \times 3 \text{ conv}  \\ \end{bmatrix} $\times$ 24  \\ \hline
\multirow{2}{*}{Transition Layer 3}   & 12 $\times$ 12 $\times$ 4                 & 1 $\times$ 1 $\times$ 1 conv                                                                                       \\ \cline{2-3} 
                                      & 6 $\times$ 6 $\times$ 2                   & 2 $\times$ 2 $\times$ 2 average pool, stride 2                                                                     \\ \hline
Dense Block 4                         & 6 $\times$ 6 $\times$ 2                   & \begin{bmatrix} 1\times 1\times 1 \text{ conv}  \\ 3 \times 3 \times 3 \text{ conv}  \\ \end{bmatrix} $\times$ 16  \\ \hline
\multirow{2}{*}{Classification Layer} & 1 $\times$ 1 $\times$ 1                   & 7 $\times$ 7 $\times$ 7 global average pool                                                                        \\ \cline{2-3} 
                                      & \multicolumn{1}{l|}{} & \begin{tabular}[c]{@{}c@{}}1000D fully-connected, \\ softmax\end{tabular}                                                   \\ \hline \hline
\end{tabular}
}
\end{table}

==> table/eval_confusionmat.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\caption{Confusion matrix for classification of test data set}
\label{tab:eval_confusionmat}
\begin{tabular}{clcc}
                                                                                                          &                                        & \multicolumn{2}{c}{\textbf{Ground-Truth Class}}                                                                                                                                                                   \\ \cline{3-4} 
                                                                                                          & \multicolumn{1}{l|}{\textbf{}}         & \multicolumn{1}{c|}{\textbf{Positive}}                                                                  & \multicolumn{1}{c|}{\textbf{Negative}}                                                                  \\ \cline{2-4} 
\multicolumn{1}{c|}{}                                                                                     & \multicolumn{1}{l|}{\textbf{Positive}} & \multicolumn{1}{c|}{\cellcolor[HTML]{8BE8BD}\begin{tabular}[c]{@{}c@{}}True Positive\\ 31\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EF6D6D}\begin{tabular}[c]{@{}c@{}}False Positive\\ 4\end{tabular}} \\ \cline{2-4} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Predicted\\ Class\end{tabular}}}} & \multicolumn{1}{l|}{\textbf{Negative}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EF6D6D}\begin{tabular}[c]{@{}c@{}}False Negative\\ 5\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{8BE8BD}\begin{tabular}[c]{@{}c@{}}True Negative\\ 55\end{tabular}} \\ \cline{2-4} 
\end{tabular}
\end{table}

==> table/eval_confusionmat1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\caption{Confusion matrix for classification of test data set}
\label{tab:eval_confusionmat}
\begin{tabular}{clcc}
                                                                                                          &                                        & \multicolumn{2}{c}{\textbf{Ground-Truth Class}}                                                                                                                                                                   \\ \cline{3-4} 
                                                                                                          & \multicolumn{1}{l|}{\textbf{}}         & \multicolumn{1}{c|}{\textbf{Positive}}                                                                  & \multicolumn{1}{c|}{\textbf{Negative}}                                                                  \\ \cline{2-4} 
\multicolumn{1}{c|}{}                                                                                     & \multicolumn{1}{l|}{\textbf{Positive}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}True Positive\\ 31\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}False Positive\\ 4\end{tabular}} \\ \cline{2-4} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Predicted\\ Class\end{tabular}}}} & \multicolumn{1}{l|}{\textbf{Negative}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}False Negative\\ 5\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}True Negative\\ 55\end{tabular}} \\ \cline{2-4} 
\end{tabular}
\end{table}

==> table/inference_eval.tex <==
\begin{table}[]
\caption{Runtime of the enhancement AI inference}
\label{tab:infer_eval}
\scalebox{0.92}{
\begin{threeparttable}
\begin{tabular}{|l|l|r|r|}
\hline
Platform                                                              & No. of cores           & Frequency & \begin{tabular}[c]{@{}l@{}}Runtime \\ (Seconds)\end{tabular} \\ \hline
NVIDIA$^{\circledR}$ V100                                                           & 5120 CUDA$^{\circledR}$ cores        & 1380 MHz  & 0.11                                                         \\ \hline
NVIDIA$^{\circledR}$ P100                                                           & 3584 CUDA$^{\circledR}$ cores        & 1328 MHz  & 0.26                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}AMD Radeon\texttrademark \\ Vega GFX 900\end{tabular}     & 4096 stream processors & 1600 MHz  & 0.27                                                         \\ \hline
NVIDIA$^{\circledR}$ T4                                                             & 2560 CUDA cores        & 1590 MHz  & 0.33                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}Intel$^{\circledR}$ Xeon$^{\circledR}$ \\ Gold 6128 CPU\end{tabular}   & 24 CPU cores           & 3400 MHz  & 1.64                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}Intel$^{\circledR}$ Arria 10\\ GX 1150 FPGA\end{tabular} & 2 compute units\tnote{*}      & 184 MHz   & 16.74                                                        \\ \hline
\end{tabular}
\begin{tablenotes}\footnotesize
\item[*]Two compute units generated using \_\_attribute\_\_((num\_compute\_units(2)) which is a  vendor-specific attribute 
\end{tablenotes}
\end{threeparttable}
}
\end{table}

==> table/inference_eval_updated.tex <==
\begin{table}[]
\caption{Runtime of the enhancement AI inference}
\label{tab:infer_eval}
\scalebox{0.76}{
\begin{threeparttable}
\begin{tabular}{|l|l|r|r|r|}
\hline
\textbf{Platform}                                                     & \textbf{\#cores} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Max.\\ Frequency\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}PyTorch \\ Runtime\\ (Sec.)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}OpenCL \\ Runtime\\ (Sec.)\end{tabular}}} \\ \hline
NVIDIA$^{\circledR}$ V100                                                           & 5120 CUDA$^{\circledR}$ cores                & 1380 MHz                                                                               & 0.22                                                                                             & 0.11                                                                                           \\ \hline
NVIDIA$^{\circledR}$ P100                                                           & 3584 CUDA$^{\circledR}$ cores                & 1328 MHz                                                                               & 0.73                                                                                            & 0.26                                                                                           \\ \hline
\begin{tabular}[c]{@{}l@{}}AMD Radeon\texttrademark\\ Vega GFX 900\end{tabular}     & 4096 stream processors         & 1600 MHz                                                                               & \color{red}$\times$                                                                                           & 0.27                                                                                           \\ \hline
NVIDIA$^{\circledR}$ T4                                                             & 2560 CUDA$^{\circledR}$ cores                & 1590 MHz                                                                               & 1.29                                                                                             & 0.33                                                                                           \\ \hline
\begin{tabular}[c]{@{}l@{}}Intel$^{\circledR}$ Xeon$^{\circledR}$\\ Gold 6128 CPU\end{tabular}   & 24 CPU cores                   & 3400 MHz                                                                               & 5.52                                                                                            & 1.64                                                                                           \\ \hline
\begin{tabular}[c]{@{}l@{}}Intel$^{\circledR}$ Arria 10\\ GX 1150 FPGA\end{tabular} & 2 compute units\tnote{*}                & 184 MHz                                                                                & \color{red}$\times$                                                                                           & 16.74                                                                                          \\ \hline
\end{tabular}
\begin{tablenotes}\footnotesize
\item[*]Two compute units generated using vendor-specific attribute, \_\_attribute\_\_((num\_compute\_units(2)) 
\item(\textcolor{red}{$\times$}):~Our implementation in PyTorch is not portable on this platform. 
\end{tablenotes}
\end{threeparttable}
}
\end{table}

==> table/kernel_event_time.tex <==
\begin{table}[]
\caption{Event-based time of the OpenCL kernels for enhancement AI inference}
\label{tab:event_eval}
\scalebox{0.90}{
\begin{tabular}{|l|r|r|r|}
\hline
\multirow{2}{*}{\textbf{Platform}} & \multicolumn{3}{c|}{\textbf{Kernel runtime (seconds)}}                \\ \cline{2-4} 
                        & \textbf{Convolution} & \textbf{Deconvolution} & \textbf{Other kernels} \\ \hline
NVIDIA$^{\circledR}$ V100                    & 0.036       & 0.059         & 0.004         \\ \hline
NVIDIA$^{\circledR}$ P100                    & 0.081       & 0.184         & 0.006         \\ \hline
\begin{tabular}[c]{@{}l@{}}AMD Radeon\texttrademark \\ Vega GFX 900\end{tabular}                  & 0.083       & 0.172         & 0.005         \\ \hline
NVIDIA$^{\circledR}$ T4                      & 0.138       & 0.171         & 0.018         \\ \hline
\begin{tabular}[c]{@{}l@{}}Intel$^{\circledR}$ Xeon$^{\circledR}$ \\ Gold 6128 CPU\end{tabular}                   & 0.495       & 1.078         & 0.057         \\ \hline
\begin{tabular}[c]{@{}l@{}}Intel$^{\circledR}$ Arria 10\\ GX 1150 FPGA\end{tabular}                & 9.819       & 2.839         & 3.991         \\ \hline
\end{tabular}}
\end{table}


==> table/training_eval_updated.tex <==
\begin{table}[]
\caption{Runtime for the enhancement AI training for 50 epochs}
\label{tab:training_eval}
\begin{threeparttable}
\begin{tabular}{|r|r|r|r|r|}
\hline
\textbf{\#Nodes\tnote{*}} & \textbf{Batch size} & \multicolumn{1}{l|}{\textbf{\#Epochs}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Training\\ Runtime\\ (hh:mm:ss)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}r@{}}MS-SSIM\\ (Avg.)\end{tabular}} \\ \hline
1                & 1                   & 50                                     & 15:14:46                                                                                              & 98.71\%                                                           \\ \hline

4                & 8                   & 50                                     & 2:27:49                                                                                               & 96.35\%                                                           \\ \hline
4                & 8                   & 100                                    & 4:58:52                                                                                                   & 96.30\%                                                                \\ \hline
4                & 16                  & 50                                     & 2:07:58                                                                                               & 95.18\%                                                           \\ \hline
8                & 8                   & 50                                     & 2:21:49                                                                                               & 95.46\%                                                           \\ \hline
8                & 8                   & 100                                    & 4:43:26                                                                                                   & 95.78\%                                                               \\ \hline
8                & 32                  & 50                                     & 1:17:25                                                                                               & 92.04\%                                                           \\ \hline
8                & 64                  & 50                                     & 1:12:24                                                                                               & 88.02\%                                                           \\ \hline
\end{tabular}
\begin{tablenotes}\footnotesize
\item[*]Each node has one NVIDIA$^{\circledR}$ T4 GPU
\item (hh:mm::ss)=(hours:minutes:seconds)
\end{tablenotes}
\end{threeparttable}
\vspace{-9pt}
%\vspace{-1cm}
\end{table}

==> table/traning_eval.tex <==
\begin{table}[]
\caption{Runtime for the enhancement AI training for 50 epochs}
\label{tab:training_eval}
\begin{threeparttable}

\begin{tabular}{|r|r|r|r|}
\hline
\#Nodes\tnote{*} & \begin{tabular}[c]{@{}l@{}}Batch size \\ per GPU\end{tabular} & \begin{tabular}[c]{@{}l@{}}Training\\ Runtime\end{tabular} & \begin{tabular}[c]{@{}l@{}}MS-SSIM\\ (Avg.)\end{tabular} \\ \hline
1       & 1                                                             & 15:14:46                                                   & 98.40\%                                                  \\ \hline
2       & 4                                                             & 4:00:31                                                    & 95.58\%                                                  \\ \hline
4       & 4                                                             & 2:07:58                                                    & 94.75\%                                                  \\ \hline
8       & 4                                                             & 1:17:25                                                    & 92.90\%                                                  \\ \hline
8       & 8                                                             & 1:12:24                                                    & 87.47\%                                                  \\ \hline
\end{tabular}
\begin{tablenotes}\footnotesize
\item[*]Each node has one NVIDIA$^{\circledR}$ T4 GPUs
\end{tablenotes}
\end{threeparttable}
%\vspace{-1cm}
\end{table}
